Improved Learning of Molecular Energetics Through an Electron-Wise Joint Charge Density and Energy Objective

We present a graph neural network-based learning framework trained to jointly predict electron densities and molecular energies. The model is trained to predict electron densities calculated with a Generalized Gradient Approximation (GGA) functional while simultaneously learning to predict molecular energies obtained with hybrid functional calculations at the B3LYP level of theory. Our results indicate that the rich spatial information in electron density distribution can be used to improve and accelerate the learning of accurate energies. By sharing an equivariant molecular representation across density and energy prediction heads, the model learns complementary molecular quantities within a unified framework. This provides a new promising route for practical use cases of many recent charge density learning frameworks for atomic scale simulations.

==> preliminary_ideas.tex <==
% We hypothesize that the energy map learns to correct for the PBE level of theory, instead of having to learn the whole map from graph/molecule to energy

==> sec/5_discussion.tex <==




